Stochastic collocation on unstructured multivariate meshes

Collocation has become a standard tool for approximation of parameterized systems in the uncertainty quantification (UQ) community. Techniques for least-squares regularization, compressive sampling recovery, and interpolatory reconstruction are becoming standard tools used in a variety of applications. Selection of a collocation mesh is frequently a challenge, but methods that construct geometrically "unstructured" collocation meshes have shown great potential due to attractive theoretical properties and direct, simple generation and implementation. We investigate properties of these meshes, presenting stability and accuracy results that can be used as guides for generating stochastic collocation grids in multiple dimensions.

==> content/setup.tex <==
\section{Stochastic Collocation}
The determination of $\widehat{c}_n(x)$ in \eqref{eq:u-ansatz} is the main difficulty, and one way to proceed is to ask that at some predetermined realizations $\left\{ z_m \right\}_{m=1}^M$ of $Z$, the ansatz match the actual response:
\begin{align}\label{eq:collocation-conditions}
  u_N(x, z_m) &\approx u(x, z_m), & m&= 1,\ldots, M,
\end{align}
where the approximation $\approx$ and the relation between $N$ and $M$ are discussed later. This is a stochastic collocation approach and is \textit{non-intrusive}: we need to compute $u(x, z_m)$, but this is accomplished by simply setting $Z = z_m$ in \eqref{eq:parameterzed-model-problem} and solving $M$ realizations of the model equation. Therefore, existing deterministic solvers can be utilized. This ability to reuse existing solvers is one of the major strengths of non-intrusive (in particular, collocation) strategies.

In contrast, \textit{intrusive} methods generally require a nontrivial mathematical reformulation of the model \eqref{eq:parameterized-model-problem}, and usually necessitate novel algorithm development. One popular intrusive method for gPC is the stochastic Galerkin approach, where $u_N$ is specified by imposing that some probabilistic moments of the model equation residual vanish. Because these moment equations are coupled and are a novel formulation compared to the original type of equation, existing deterministic solvers of \eqref{eq:parameterized-model-problem} cannot be used. The advantage of intrusive methods compared to non-intrusive methods is that one can usually make more formal mathematical statements about convergence of $u_N$ with an intrusive formulation. For details of intrusive methods, see \cite{Ghanem,}. Although intrusive methods are advantageous in many situations, in this paper we only consider non-intrusive collocation approaches.

The focus of this paper discusses how to enforce the collocation conditions \eqref{eq:collocation-conditions}. We investigate three situations:
\begin{itemize}
  \item $M = N$: with an equal number of linear constraints and degrees of freedom, we may enforce interpolation
  \item $M > N$: when there are more constraints than degrees of freedom, we employ regression to attain a solution
  \item $M < N$: with more degrees of freedom than constraints, we may seek sparse solutions and appeal to the theory of compressive sampling
\end{itemize}

Examples of sampling strategies that we consider as `structured' are tensor-product constructions and sparse grid constructions. The former is quickly seen as infeasible for large dimensionality $d$. If we have an $m$-point one-dimensional grid (such as a Clenshaw-Curtis grid), then an isotropic tensorization has $M = m^d$ samples; this exponential dependence on $d$ is usually not computationally acceptable.

Sparse grids are unions of anistropically-tensorized grids, and have proven very effective
\cite{FabioC3,bungartz_sparse_2004,gerstner_numerical_1998,barthelmann_high_2000} at approximating high-dimensional problems. However, the sparse grids' adherence to rigid and predictable layouts have the potential weakness of `missing' important features that do not line up with cardinal directions or coordinates in multivariate space. Additionally, isotropic sparse grids are usually used at early stages of computations to determine important directions. Unfortunately, most isotropic sparse grid constructions cluster nodes around the cardinal axes, which occuply a small region in multivariate space. Thus it is possible that most of parameter space $D$ will not be sampled until much later in the procedure, if at all. We believe that unstructured sample designs have the ability to mitigate these shortcomings.

%briefly present two collocation strategies that we consider `structured' in the sense explained in the introduction.
%\subsection{Tensor product constructions}
%One of the most simple methods to construct multivariate meshes is to use one-dimensional grids to construct a tensor-product mesh. If $N_1, \ldots N_d$ grid points are used in each of dimensions $1, \ldots, d$, respectively, then the tensor-product mesh has $\prod_{j=1}^d N_j$ total points. It is clear that the cardinality of a tensor-product meshes grows exponentially with the dimension $d$. %and a tensor-product mesh quickly becomes infeasible for moderately large dimension $d$.
%
%The advantage of tensor-product constructions is that many univariate results concerning accuracy and stability can be extended to multivariate settings (CITE). However, the curse of dimensionality here quickly renders this direct approach infeasible.
%
%\subsection{Sparse grids}
%A Smolyak sparse grid is a union of tensor-product meshes. However, the meshes are chosen in a way that attempts to mitigate the exponential dependence on dimension. The original construction is due to Smolyak (CITE) but modern sparse grid variants are significantly more sophisticated than this original work.
%
%For $k=0, 1,\ldots$, we define $\Theta^j_k$ as one-dimensional grids for dimension $j$. Then a multivariate sparse grid of level $\ell$ is given by
%\begin{align*}
%  \Theta_{\ell} = \bigcup_{|\alpha| \leq \ell} \bigotimes_{j=1}^d \Theta^j_{\alpha_j}.
%\end{align*}
%One may define the $\Theta^j_k$ in any manner, but a popular example is taking identical $\Theta^j_k$ meshes for each dimension as the $2^k+1$-size Chebyshev Gauss-Lobatto mesh:
%\begin{align*}
%  \Theta^j_k = \left\{\cos \left( \frac{(n-1)\pi}{2^k} \right)\right\}_{n=1}^{2^k}
%\end{align*}
%These univariate rules are nested, i.e., $\Theta^j_k \subset \Theta^j_{k+1}$, and the sparse grid construction $\Theta_{\ell}$ inherits this nestnedness property. Thus refinement may proceed simply by adding samples to the existing grid. This allows one to easily implement adaptive refinement algorithms based on grid hierarchical surpluses. (CITE)
%
%Other proposed grids for the univarite composite rules involve Gauss-Patterson rules (CITE) and Leja sequences (CITE), but the basic idea for the multivariate construction is the same. In addition, one need not use global basis functions and instead may use e.g. local polynomial functions. Convergence can be stated by appealing to smoothness arguments with multidimensional Sobolev norms. (CITE)
%
%Sparse grids are simple, effective, and have been used to great effect. However, the sparse grids' adherence to rigid and predictable layouts have the potential weakness of 'missing' important features that do not line up with cardinal directions or coordinates in multivariate space. Additionally, isotropic sparse grids are usually used at early stages of computations to determine important directions. Unfortunately, most isotropic sparse grid constructions cluster nodes around the cardinal axes, which occuply a small region in multivariate space. Thus it is possible that most of parameter space $\Omega$ will not be sampled until much later in the procedure, if at all. We believe that unstructured sample designs have the ability to mitigate these shortcomings.
%(Mention sparse grid weaknesses here...why we want to explore other things.)

%\subsection{Unstructured grids}
%The focus of this paper is on unstructured grids, in contrast to tensor-product and sparse grids. In essence, most other

